GraphScope Flex: LEGO-like Graph Computing Stack

Graph computing has become increasingly crucial in processing large-scale graph data, with numerous systems developed for this purpose. Two years ago, we introduced GraphScope as a system addressing a wide array of graph computing needs, including graph traversal, analytics, and learning in one system. Since its inception, GraphScope has achieved significant technological advancements and gained widespread adoption across various industries. However, one key lesson from this journey has been understanding the limitations of a "one-size-fits-all" approach, especially when dealing with the diversity of programming interfaces, applications, and data storage formats in graph computing. In response to these challenges, we present GraphScope Flex, the next iteration of GraphScope. GraphScope Flex is designed to be both resource-efficient and cost-effective, while also providing flexibility and user-friendliness through its LEGO-like modularity. This paper explores the architectural innovations and fundamental design principles of GraphScope Flex, all of which are direct outcomes of the lessons learned during our ongoing development process. We validate the adaptability and efficiency of GraphScope Flex with extensive evaluations on synthetic and real-world datasets. The results show that GraphScope Flex achieves 2.4X throughput and up to 55.7X speedup over other systems on the LDBC Social Network and Graphalytics benchmarks, respectively. Furthermore, GraphScope Flex accomplishes up to a 2,400X performance gain in real-world applications, demonstrating its proficiency across a wide range of graph computing scenarios with increased effectiveness.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all: paper

paper: paper.pdf
.PHONY: paper

paper.pdf:
	pdflatex -interaction=nonstopmode paper.tex || true
	- bibtex paper.aux
	pdflatex -interaction=nonstopmode paper.tex || true
	pdflatex -interaction=nonstopmode paper.tex
.PHONY: paper.pdf

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux *.fdb_latexmk \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \



clean: docclean
	# $(RM)  $(PACKAGE).cls 
	

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sec-rel.tex <==
\section{Related Work}
\label{sec:related-work}

\stitle{Graph Storages.} 
\eat{There exist diverse types of graph storage, and they often make different assumptions and target different use cases.
 For instance, some~\cite{macko2015llama, terrace, dhulipala2019low} presume that graph data updates occur in batches without the need for transactions. 
 Conversely, some~\cite{zhu13livegraph, Sortledton, de2021teseo, ediger2012stinger, kumar2020graphone} are designed for graphs that get updated frequently under transactional guarantees. 
 In addition, some work~\cite{han2010igraph, gedik2014disk, han2013turbograph} are designed to support disk-based storage.
 Thus, no graph storage can provide optimal performance under all cases.
  In addition, different types of graph storage usually offer different interfaces for graph computation engines. 
  When attempting to make a computation engine work on different storage, developers need to manually write a wrapper program or data transformation program for new storage. 
  In \gsf, we provide unified graph retrieval interfaces for both graph storage and computation engines to avoid such manual-intensive work.}
Graph storage types differ, each designed for specific uses and assumptions. Some work \cite{macko2015llama, terrace, dhulipala2019low} handle batch graph data updates without needing transactions, while others \cite{zhu13livegraph, Sortledton, de2021teseo, ediger2012stinger, kumar2020graphone} support frequently updated graphs with transactional guarantees. In addition, some work \cite{han2010igraph, gedik2014disk, han2013turbograph} focus on disk-based storage. Therefore, no single storage solution is universally optimal. Different storage types also mean diverse computation engine interfaces, often necessitating manual wrapper or data transformation program development. \gsf~ addresses this by offering a unified interface with various storage backends, catering to diverse storage needs and reducing manual effort.

\stitle{Graph Engines.}
The applications of graphs are highly diverse, and consequently, various graph engines have been developed for different scenarios. 
 Typically, these engines are designed to handle a particular type of graph computation. 
 For instance, while some are created for general-purpose graph analytics~\cite{zhu2016gemini, fan2018parallelizing, chen2019powerlyra, vora2019lumos}, others are built for graph analytics on GPUs~\cite{wang2017gunrock, Ben2017Groute, gum, pandey2020c}, graph interactive queries~\cite{glogs, qian2021gaia, trigonakis2021adfs, jamshidi2020peregrine}, or GNN~\cite{gandhi2021p3, yang2022gnnlab, liu2023bgl}. 
Further, there exists some work which attempts to bridge graph computation with other domains. 
For instance, GraphX~\cite{graphx} is designed to support graph processing within the Spark ecosystem, GART~\cite{gart} is dedicated to bridging relational databases and graph computation. %and Gunrock~\cite{wang2017gunrock}, Groute~\cite{Ben2017Groute} and GUM~\cite{gum} depend on GPUs to accelerate graph processing. 
Different graph engines necessitate different dependencies, programming languages, and hardware, which makes deploying multiple engines challenging. 
However, the modular architecture of \gsf~enables the deployment of graph engines on demand, thereby enhancing deployment flexibility and user experience.

\stitle{Graph Applications.}
Users often utilize programming models or high-level query languages supported by graph engines to write a graph application. 
Unlike domains like relational database where SQL is the de facto 
standard, these programming models and query languages for graphs are highly varied, providing users with several choices even for the same type of graph applications. 
To illustrate, various models excel at representing graph analytics applications (\eg the vertex-centric model~\cite{malewicz2010pregel}, block-centric model~\cite{tian2013think}, edge-centric model~\cite{roy2013x}, GAS~\cite{gonzalez2012powergraph}, PIE~\cite{fan2018parallelizing}, GraphBLAS~\cite{graphblas} and FLASH~\cite{li2023flash}). 
%The vertex-centric model~\cite{malewicz2010pregel} effectively expresses message passing-like algorithms. PIE~\cite{fan2018parallelizing} is adept at conveying sequential graph algorithms. GraphBLAS~\cite{graphblas} is proficient in demonstrating algorithms using linear algebra. Lastly, FLASH~\cite{li2023flash} excels at illustrating algorithms that involve beyond-neighborhood communication.
\gsf~manages this diversity by supporting a range of programming models and query languages, to facilitate easy usage for users.

